PLATINUM: Semi-Supervised Model Agnostic Meta-Learning using Submodular Mutual Information

Few-shot classification (FSC) requires training models using a few (typically one to five) data points per class. Meta learning has proven to be able to learn a parametrized model for FSC by training on various other classification tasks. In this work, we propose PLATINUM (semi-suPervised modeL Agnostic meTa-learnIng usiNg sUbmodular Mutual information), a novel semi-supervised model agnostic meta-learning framework that uses the submodular mutual information (SMI) functions to boost the performance of FSC. PLATINUM leverages unlabeled data in the inner and outer loop using SMI functions during meta-training and obtains richer meta-learned parameterizations for meta-test. We study the performance of PLATINUM in two scenarios - 1) where the unlabeled data points belong to the same set of classes as the labeled set of a certain episode, and 2) where there exist out-of-distribution classes that do not belong to the labeled set. We evaluate our method on various settings on the miniImageNet, tieredImageNet and Fewshot-CIFAR100 datasets. Our experiments show that PLATINUM outperforms MAML and semi-supervised approaches like pseduo-labeling for semi-supervised FSC, especially for small ratio of labeled examples per class.

==> section_tex_files/formulation_2.tex <==
Reference of Jamboard:

\url{https://jamboard.google.com/d/1LXMEC4MBCY_RRWtzHYPd2Extd77WGAS7sD2TkbgXt84/edit?usp=sharing}

Assume the total number of tasks during training is $T$. Namely we have the training tasks $\{(\mathcal{S}_i, \mathcal{Q}_i, \mathcal{U}_i)\}_{i=1}^{T}$. Define $L(\theta, S) = \sum_{i\in S}L(\theta, x^i, y^i)$ as the loss on a set $S$ of instances. Denote $L$ as the training loss, $L_V$ as the validation loss (i.e., $L_V(\phi, \mathcal{Q})$ as the loss on the validation (query) set $\mathcal{Q}$). $\theta$ is meta-parameter, and $\phi_i$ is adapted model parameter. $B$ is the budge size of selected samples.

The goal is to select $\mathcal{A}_i = \{{x}_1, {x}_2, ..., {x}_m\}$ from $\mathcal{U}_i$ for each task $i$, $|\mathcal{A}_i|\leq B$, such that the model trained on $\{\mathcal{A}_i, \mathcal{S}_i\}$ for task $i$ will perform well on the corresponding query (validation) set $\mathcal{Q}_i$.

The optimization objective is:
\begin{equation}
\label{optim}
    \min_{\theta, \{\mathcal{A}_i\}_{i=1}^{T}, |\mathcal{A}_i\leq B|} \sum_{i=1}^{T} L_V(\phi_i, \mathcal{Q}_i) - \lambda \sum_{i=1}^{T}\mathcal{I}_f(\mathcal{A}_i; \mathcal{Q}_i)
\end{equation}

s.t.:

for each task $i$ (consider each task separately), $\phi_i$ satisfies:
    \begin{equation}
    \begin{aligned}
        \phi_i &= \argmin_{\phi_i} L_{ssl}(\theta, (\mathcal{A}_i, \mathcal{S}_i))
    \end{aligned}
    \end{equation}

\begin{equation}
\label{Ai}
\mathcal{A}_i = \argmin_{\mathcal{A}_i, |\mathcal{A}_i\leq B|} L_V(\phi_i, \mathcal{Q}_i) - \lambda \mathcal{I}_f(\mathcal{A}_i; \mathcal{Q}_i)   
\end{equation}

where $\lambda > 0$, and $\mathcal{I}_f(\mathcal{A}_i;\mathcal{Q}_i)$ is the submodular mutual information (SMI). Maximizing SMI will select points similar to $\mathcal{Q}_i$ while being diverse.

\textbf{How to Optimize Equation~(\ref{optim})}:

Let 
\begin{equation}
    L_{ssl}(\theta, (\mathcal{A}_i, \mathcal{S}_i)) = L({\theta}, \mathcal{S}_i) {\color{red} - \alpha \sum_{j\in \mathcal{A}_i} r(\theta, x_j)}
\end{equation}

$L({\theta}, \mathcal{S}_i)$ is the Cross-Entropy loss for labeled support set. The \textcolor{red}{second red term} is the loss for unlabeled set.

If only one step gradient is considered:
\begin{equation}
\begin{aligned}
\phi_i &= \argmin_{\phi_i} L_{ssl}(\theta, (\mathcal{A}_i, \mathcal{S}_i)) \\
    &= {\theta} - \alpha \nabla_{{\theta}}L_{ssl}({\theta}, (\mathcal{A}_i ,  \mathcal{S}_i)) \\
    &= {\theta} - \alpha \nabla_{{\theta}}L({\theta}, \mathcal{S}_i) {\color{red} - \alpha \sum_{j\in \mathcal{A}_i} \nabla_{\theta} r(\theta, x_j)}
\end{aligned}
\end{equation}

For the iteration $t$:

\begin{equation}
\label{Ai}
\begin{aligned}
\mathcal{A}_i^t &= \argmin_{\mathcal{A}_i, |\mathcal{A}_i\leq B|} L_V(\phi_i^t, \mathcal{Q}_i) - \lambda \mathcal{I}_f(\mathcal{A}_i; \mathcal{Q}_i) \\   
 &= \argmin_{\mathcal{A}_i, |\mathcal{A}_i\leq B|} L_V({\theta}^t - \alpha \nabla_{{\theta}}L({\theta}, \mathcal{S}_i) {\color{red} - \alpha \sum_{j\in \mathcal{A}_i} \nabla_{\theta} r(\theta, x_j)}, \mathcal{Q}_i) - \lambda \mathcal{I}_f(\mathcal{A}_i; \mathcal{Q}_i) \end{aligned}  
\end{equation}



Equation~(\ref{Ai}) tries to select a subset $\mathcal{A}_i$ of the unlabeled set $\mathcal{U}_i$, such that the loss on the validation (query) set $\mathcal{Q}_i$ is minimized. We can replace the loss function $L_V$ and $L$ with log-likelihood functions $LL_V$ and $LL$ in which case, the argmin becomes argmax:

\begin{equation}
\label{Ai-argmax}
\mathcal{A}_i^t = \argmax_{\mathcal{A}_i, |\mathcal{A}_i\leq B|} LL_V({\theta}^t - \alpha \nabla_{{\theta}}LL({\theta}, \mathcal{S}_i) {\color{red} - \alpha \sum_{j\in \mathcal{A}_i} \nabla_{\theta} r(\theta, x_j)}) + \lambda \mathcal{I}_f(\mathcal{A}_i; \mathcal{Q}_i)   
\end{equation}

In fact, we can proof that:
\begin{equation}
\label{lvig}
        L_V({\theta}^t - \alpha \nabla_{{\theta}}L({\theta}, \mathcal{S}_i) {\color{red} - \alpha \sum_{j\in \mathcal{A}_i} \nabla_{\theta} r(\theta, x_j)}, \mathcal{Q}_i) \approx - \mathcal{I}_g(\mathcal{A}_i; \mathcal{S}_i)
\end{equation}
with some set function $g$.


Notes: 

0. How to prove: equation (\ref{lvig})?

1. The \textcolor{red}{second red term} is the loss for unlabeled set, which depends on the specific SSL algorithm.

2. The current formulation and optimization is a jointing optimization manner. How about the two independent stages (selection of $\mathcal{A}$ and MAML)? 

3. To avoid the huge number of $T$, in practice, a model is usually trained through a ``batch'' manner. So this should not have a big problem.

4. If this is not a few shot learning problem, and we do not consider MAML, after the optimization, we will output the model parameters $\phi$. $\phi$ will be used directly during test phase without any learning process again.

5. The other option to optimize $\phi_i$ is to consider all tasks together. (not the focus.)
\begin{equation}
    \phi_1, \phi_2, ..., \phi_T = \argmin_{\theta}\sum_{i}^{T} L(\theta, (\mathcal{A}_i,\mathcal{S}_i)) + \Omega(\theta)
\end{equation}

% \section{How to Select: Submodular Information Measure (SIM) based approach}
This section is to introduce how to select samples from the unlabeled set $\mathcal{U}_i$ via the submodular information measures from Prof.Iyer's recent paper.

The algorithm is shown in Algorithm~\ref{alg-ssl-fsl}.Some details could be found from Prof.Iyer's paper. i.e., the instantiations of SIM, definition of similarity matrix, etc.

Notes:

1. For SMI, or SCG, we just need to do some modification according to the Table.1 from Prof.Iyer's paper.

2. The loss $\mathcal{H}$ shown in the algorithm should be the same to $L$, could it be cross entropy loss?

3. If we only consider the imbalance, and OOD scenario, which means we might only consider SMI through the setting: $\mathcal{Q} \leftarrow \mathcal{Q}, \mathcal{P} \leftarrow \emptyset $. \textcolor{blue}{So in this case, the query set in meta-learning will be viewed as the $\mathcal{Q}_i$ in SIM-based approach.}

\begin{algorithm}[t]
\small
\caption{SIM-based SSL for few shot learning}
\begin{algorithmic}[1]
\label{alg-ssl-fsl}
\REQUIRE Training tasks: $\mathcal{T}_{tr}=\{\mathcal{S}_i,\mathcal{Q}_i, \mathcal{U}_i\}_{i=1}^{T}$, Loss function $\mathcal{H}$ for learning model $\mathcal{M}$, Batch size of tasks: $b$, Budge of selected samples from unlabeled set: B

% \REQUIRE $\epsilon$ \hspace{0.1cm} Gradient clipping threshold parameter
\STATE Randomly initialize $\boldsymbol{\theta}$
\WHILE{not done}
\STATE Sample mini-batch of tasks $\{\mathcal{S}_i,\mathcal{Q}_i, \mathcal{U}_i\}_{i=1}^{b} \sim \mathcal{T}_{tr}$
\FOR{each task $\mathcal{T}_i=\{\mathcal{S}_i,\mathcal{Q}_i, \mathcal{U}_i\},\forall i\in [1,b]$ }
\STATE Compute adapted parameters $\phi_i$ with gradient descent by Eq.~(\ref{param-adaptation}) [namely Eq.(\ref{param-adaptation-ssl})]

\STATE Using model parameters $\phi_i$, compute gradients using hypothesized labels $
\left\{\nabla_{\theta} \mathcal{H}\left(\tilde{x}_{j}, \hat{y}_{j}, \theta\right), \forall j \in \mathcal{U}\right\}
$, and obtain a similarity matrix $X$.
\STATE Instantiate a submodular function $f$ based on $X$.
\STATE $
\mathcal{A}_{i} \leftarrow \operatorname{argmax}_{\mathcal{A}_i \subseteq \mathcal{U}_i,|\mathcal{A}_i| \leq B} I_{f}(\mathcal{A}_i; \mathcal{Q}_i \mid \mathcal{P}_i)
$ (Optimize SCMI with an appropriate choice of $\mathcal{Q}_i$ and $\mathcal{P}_i$, see Table.1 in Prof.Iyer's paper)
% \STATE Get labels $L(\mathcal{A}_i)$ for selected samples $\mathcal{A}_i$, and form a new support set $(\mathcal{A}_i,L(\mathcal{A}_i))\cup \mathcal{S}_i$
\STATE Update model parameters from $\phi_i$ to $\phi_i'$ via Eq.(\ref{st1})
\ENDFOR

//\textit{meta update}
\STATE Update $\boldsymbol{\theta}^{(t+1)}$ by Eq.~(\ref{meta-update}) using $\{\mathcal{Q}_i\}_{i=1}^{b}$
\ENDWHILE
\STATE Return the model initialization $\theta$.
\end{algorithmic}
\end{algorithm}


==> section_tex_files/formulation_backup.tex <==
Assume the total number of tasks during the training is $T$. Namely we have the training tasks $\{(\mathcal{S}_i, \mathcal{Q}_i, \mathcal{U}_i)\}_{i=1}^{T}$.

The goal of the proposed approach is to obtain the optimal initial parameters that minimize the meta-training objective:
\begin{equation}
\begin{aligned}
    \label{meta-objective-ssl}
    \overbrace{\boldsymbol{\theta}^*= \argmin_{\boldsymbol{\theta} \in \boldsymbol{\Theta}}{\mathcal{F}(\boldsymbol{\theta})}}^{outer-level}\text{\hspace{1.7cm}}\\
    \text{where, }\mathcal{F}(\boldsymbol{\theta}) = \frac{1}{M}\sum_{i=1}^{M}L_V(\overbrace{\color{blue}\mathcal{A}lg(\boldsymbol{\theta}, (\mathcal{S}_{i},\mathcal{U}_i))}^{inner-level}, \mathcal{Q}_{i})\text{\hspace{0.5cm}}
\end{aligned}
\end{equation}

As mentioned previously, for MAML, $\mathcal{A}lg(\boldsymbol{\theta}, \mathcal{S}_{i})$ corresponds to single or multiple gradient steps on the labeled support set. Here $\color{blue}\mathcal{A}lg(\boldsymbol{\theta}, (\mathcal{S}_{i},\mathcal{U}_i))$ corresponds to single or multiple gradient steps on the labeled support set and unlabeled set for task $i$. In case of a single gradient step, $\mathcal{A}lg(\boldsymbol{\theta}, \mathcal{S}_{i})$ can be specified as below:
\begin{equation}
    \label{param-adaptation-ssl}
    \phi_i = {\color{blue}\mathcal{A}lg(\boldsymbol{\theta}, (\mathcal{S}_{i},\mathcal{U}_i))} = \boldsymbol{\theta} - \alpha \nabla_{\boldsymbol{\theta}}L_{ssl}(\boldsymbol{\theta}, (\mathcal{S}_{i},\mathcal{U}_i))
\end{equation}

Note:

1. $L_{ssl}$ is the loss function which is commonly used in conventional semi-supervised learning, such as Pseudo-Label~\cite{lee2013pseudo} and VAT~\cite{miyato2018virtual}.

Same to MAML, the output of the model would be the optimal initialization of the model. During meta-testing for each novel task, using the initialization of the SSL model, the regular semi-supervised learning approach will be applied.


\subsection{Notation}
Some notations are listed here:
\begin{itemize}
    \item $\theta$: meta-parameters
    \item $\phi$: task specific model parameters
    \item Task $i$ in meta-training: $\mathcal{T}_i = \{\mathcal{S}_i, \mathcal{Q}_i, \mathcal{U}_i\}$
    \item Task $i$ in meta-test: $\mathcal{T}'_i = \{\mathcal{S}'_i, \mathcal{Q}'_i, \mathcal{U}'_i\}$
    \item $\mathcal{S}_i$, $\mathcal{Q}_i$, $\mathcal{U}_i$: Support set, Query set, and Unlabeled set for task $\mathcal{T}_i$ in meta-training
    \item $\mathcal{S}'_i$, $\mathcal{Q}'_i$, $\mathcal{U}'_i$: Support set, Query set, and Unlabeled set for task $\mathcal{T}'_i$ in meta-test
    \item $\mathcal{S}_{iu}$: Selected unlabeled examples from Unlabeled set for task $\mathcal{T}_i$ in the inner loop in meta-training
    \item $\mathcal{Q}_{iu}$: Selected unlabeled examples from Unlabeled set for task $\mathcal{T}_i$ in the outer loop in meta-training
    \item $L(\theta;\cdot)$: Cross entropy loss based on model with parameters $\theta$
\end{itemize}

For now, we consider subset selection in the inner loop based on Support set and subset selection in the outer loop based on Query set. Namely:
\begin{equation}
    \mathcal{S}_{iu} = \argmax_{A\subseteq \mathcal{U}_i, |A|\leq B}I_{f}(A; \mathcal{S}_i) 
\end{equation}

\begin{equation}
    \mathcal{Q}_{iu} = \argmax_{A\subseteq \mathcal{U}_i, |A|\leq B}I_{f}(A; \mathcal{Q}_i)
\end{equation}

$f$ here is the SMI function, which is FLQMI. Details could be found from Table 2.(a) in the paper~\cite{kothawade2021similar}.


\subsection{Formulation}

Meta-parameter update according to:
\begin{equation}
    \theta = \argmin_{\theta} L_{maml+SMI} = \argmin_{\theta} \mathcal{F}(\boldsymbol{\theta})
\end{equation}

The final loss function is:

\begin{equation}
\begin{aligned}
    \label{meta-objective-ssl}
    \overbrace{\boldsymbol{\theta}^*= \argmin_{\boldsymbol{\theta} \in \boldsymbol{\Theta}}{\mathcal{F}(\boldsymbol{\theta})}}^{outer-level}\text{\hspace{1.7cm}}\\
    \text{where, }\mathcal{F}(\boldsymbol{\theta}) = \frac{1}{M}\sum_{i=1}^{M}L(\overbrace{\color{blue}\phi_i}^{inner-level}, (\mathcal{Q}_{i}, \mathcal{U}_{i}))\text{\hspace{0.5cm}}
\end{aligned}
\end{equation}

$$
\phi_i = \mathcal{A}lg(\boldsymbol{\theta}, (\mathcal{S}_{i},\mathcal{U}_i)) = \operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L_{ssl}\left(\theta ; S_{iu}\right)
$$

\begin{equation}
\begin{aligned}
&{\mathcal{F}(\boldsymbol{\theta})} = \frac{1}{M}\sum_{i=1}^{M}L({\phi_i}, (\mathcal{Q}_{i}, \mathcal{U}_{i})) \\
&=\frac{1}{M}\sum_{i=1}^{M} L\left(\phi_{i} ; Q_{i}\right)+ \tau' L_{ssl}\left(\phi_{i} ; Q_{iu}\right) \\
&=\frac{1}{M}\sum_{i=1}^{M} L\left(\operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L_{ssl}\left(\theta ; S_{iu}\right) ; Q_{i}\right)+ \tau' L_{ssl}\left(\operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L_{ssl}\left(\theta ; S_{iu}\right) ; Q_{iu}\right)
\end{aligned}
\end{equation}

in which:
\begin{equation}
    \mathcal{S}_{iu} = \argmax_{A\subseteq \mathcal{U}_i, |A|\leq B}I_{f}(A; \mathcal{S}_i) 
\end{equation}

\begin{equation}
    \mathcal{Q}_{iu} = \argmax_{A\subseteq \mathcal{U}_i, |A|\leq B}I_{f}(A; \mathcal{Q}_i)
\end{equation}



\subsection{Inner loop}

Task specific model parameters for task $\mathcal{T}_i$: 
\begin{equation}
    \begin{aligned}
\phi_{i}=& \operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L\left(\theta ; S_{iu}\right) \\
=&\theta-\alpha \nabla_{\theta} L\left(\theta ; S_{i}\right)-\alpha \tau \nabla_{\theta} L\left(\theta ; S_{iu}\right)  \text{(one step gradient update example)}
\end{aligned}
\end{equation}


In which, $\alpha$ is learning rate. $\tau$ is the coefficient from the pseudo labeling approach. Since it is an increasing temperature variable, let $\tau^{(j)}$ denote the $\tau$ in step $j$.

Since there are several gradient update steps in inner loop. Take three steps for example.

Let $\phi_{i}^{(j)}$ denote the model parameters for $j$-th step for task $T_i$.
\begin{itemize}
    \item initialization: $\phi_{i}^{(0)} = \theta$  
    \item inner step 1: 
    $$
\phi_i^{(1)}=\theta-\alpha \nabla_{\theta} L(\theta ; S_i)-\alpha \tau^{(1)} \nabla_{\theta} L\left(\theta ; S_{iu}\right)
$$

$\mathcal{S}_{iu} = \argmin_{A\subseteq \mathcal{U}_i}I_{f}(A; \mathcal{S}_i)$. In this step, the CNN model used to calculate the gradient in SMI is parameterized by {\color{blue}$\theta$}.

    \item inner step 2: 
     $$
\phi_i^{(2)}=\theta-\alpha \nabla_{\phi^{(1)}} L(\phi^{(1)} ; S_i)-\alpha \tau^{(2)} \nabla_{\phi^{(1)}} L\left(\phi^{(1)} ; S_{iu}\right)
$$

$\mathcal{S}_{iu} = \argmin_{A\subseteq \mathcal{U}_i}I_{f}(A; \mathcal{S}_i)$. In this step, the CNN model used to calculate the gradient in SMI is parameterized by {\color{blue}$\phi^{(1)}$}.

    \item inner step 3: 
     $$
\phi_i^{(3)}=\theta-\alpha \nabla_{\phi^{(2)}} L(\phi^{(2)} ; S_i)-\alpha \tau^{(3)} \nabla_{\phi^{(2)}} L\left(\phi^{(2)}; S_{iu}\right)
$$

$\mathcal{S}_{iu} = \argmin_{A\subseteq \mathcal{U}_i}I_{f}(A; \mathcal{S}_i)$. In this step, the CNN model used to calculate the gradient in SMI is parameterized by {\color{blue}$\phi^{(2)}$}.

    \item inner loop end. 
    
    Model parameters for task $T_i$ udpate process:
    
    $$\phi^{(0)} (:=\theta) \rightarrow \phi^{(1)}\rightarrow \phi^{(2)}\rightarrow \phi^{(3)}$$
    
\end{itemize}

\subsection{Outer Loop}
Meta-parameter update according to:
\begin{equation}
    \theta = \argmin_{\theta} L_{maml+SMI}
\end{equation}

The final loss function is:

\begin{equation}
\begin{aligned}
&L_{maml+SMI}=\frac{1}{M}\sum_{i=1}^{M} L\left(\phi_{i} ; Q_{i}\right)+ \tau' L\left(\phi_{i} ; Q_{iu}\right) \\
&=\frac{1}{M}\sum_{i=1}^{M} L\left(\operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L\left(\theta ; S_{iu}\right) ; Q_{i}\right)+ \tau' L\left(\operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L\left(\theta ; S_{iu}\right) ; Q_{iu}\right)
\end{aligned}
\end{equation}

in which, $T$ is the set of meta-training tasks. $\tau'$ is still a coefficient borrowed from the pseudo label formulation.

The second equal in the above equation is according to the inner loop update:
$$
\phi_i = \operatorname{argmin}_{\theta} L\left(\theta ; S_{i}\right)+\tau L\left(\theta ; S_{iu}\right)
$$


Since there is only one step in the outer loop, subset selection only happens one time.

\begin{equation}
    \mathcal{Q}_{iu} = \argmin_{A\subseteq \mathcal{U}_i}I_{f}(A; \mathcal{Q}_i)
\end{equation}
The CNN model used here should be the final model parameter after the inner loop: {\color{blue}$\phi_i^{(3)}$}.

The motivation here to use $\phi_i^{(3)}$ instead of meta-parameter $\theta$ is that SMI needs a CNN model which has powerful representation. For task $T_i$, $\phi_i^{(3)}$ is more powerful than $\theta$.

